Leveraging Passage Embeddings for Efficient Listwise Reranking with Large Language Models

Recent studies have demonstrated the effectiveness of using large language language models (LLMs) in passage ranking. The listwise approaches, such as RankGPT, have become new state-of-the-art in this task. However, the efficiency of RankGPT models is limited by the maximum context length and relatively high latency of LLM inference. To address these issues, in this paper, we propose PE-Rank, leveraging the single passage embedding as a good context compression for efficient listwise passage reranking. By treating each passage as a special token, we can directly input passage embeddings into LLMs, thereby reducing input length. Additionally, we introduce an inference method that dynamically constrains the decoding space to these special tokens, accelerating the decoding process. For adapting the model to reranking, we employ listwise learning to rank loss for training. Evaluation results on multiple benchmarks demonstrate that PE-Rank significantly improves efficiency in both prefilling and decoding, while maintaining competitive ranking effectiveness. The Code is available at https://github.com/liuqi6777/pe_rank.

==> prompts/summarize.tex <==
\begin{table}[h]
\centering
\begin{tcolorbox}[width=\linewidth]
\textbf{User:}

Summarize the following passage, only output the summary, do not include anything else.

Passage: \texttt{\{\{content\}\}}

%
\end{tcolorbox}
\caption{Prompts used for generating summary using Mistral-7B.}
\label{tab:prompt_summarize}
\end{table}

==> tables/efficiency_covid.tex <==
\begin{table}[t]
\small
\centering
\begin{tabular}{@{}l|c|ccc@{}}
\toprule
% \textbf{Model}         & \textbf{$k$} & \multicolumn{3}{c}{\textbf{TREC Covid}}                  \\
\textbf{Model}         & \textbf{$k$} & \textbf{NDCG} & \textbf{\#Proc.} & \textbf{Latency (s)} \\ \midrule
$\text{RankMistral}_p$ & \multirow{4}{*}{20} & 70.90  & \hphantom{0}8190.9 & \hphantom{0}2.51 \hphantom{($\times$.00)}  \\
$\text{RankMistral}_s$ &                     & 65.15  & \hphantom{0}2224.2 & \hphantom{0}1.92 ($\times$.76)   \\
$\text{RankMistral}_t$ &                     & 66.71  & \hphantom{00}829.7 & \hphantom{0}1.89 ($\times$.75)   \\
-                      &                     & 72.34  & \hphantom{00}344.3 & \hphantom{0}0.44 ($\times$.18)   \\ 
\midrule
$\text{RankMistral}_p$ & \multirow{4}{*}{100}& 77.80  & 71431.2            & 21.46 \hphantom{($\times$.00)}   \\
$\text{RankMistral}_s$ &                     & 73.85  & 20148.6            & 16.94 ($\times$.79) \\
$\text{RankMistral}_t$ &                     & 75.40  & \hphantom{0}7555.0 & 15.87 ($\times$.74) \\
-                      &                     & 77.72  & \hphantom{0}3098.9 & \hphantom{0}3.65 ($\times$.17)  \\ \bottomrule
\end{tabular}
\caption{}
\label{tab:efficiency_covid}
\end{table}

==> tables/efficiency_dl20.tex <==
\begin{table}[t]
\centering
\small
\begin{tabular}{@{}l|c|ccc@{}}
\toprule
{\textbf{Model}}  &         $n$          & \textbf{NDCG} & \textbf{\# Proc.}  & \textbf{Latency (s)}                      \\ \midrule
$\text{RankMistral}_p$ & \multirow{4}{*}{20}  & 60.64         & \hphantom{0}2190.4 & \hphantom{0}1.88 \hphantom{($\times$.00)} \\
$\text{RankMistral}_s$ &                      & 59.52         & \hphantom{0}1446.8 & \hphantom{0}1.81 ($\times$.97)            \\
$\text{RankMistral}_t$ &                      & 42.28         & \hphantom{00}422.8 & \hphantom{0}1.85 ($\times$.99)            \\
PE-Rank                &                      & 56.48         & \hphantom{00}327.7 & \hphantom{0}0.42 ($\times$.22)            \\ \midrule
$\text{RankMistral}_p$ & \multirow{4}{*}{100} & 68.39         & 19787.0            & 16.31 \hphantom{($\times$.00)}            \\
$\text{RankMistral}_s$ &                      & 66.14         & 13514.3            & 15.74 ($\times$.97)                       \\
$\text{RankMistral}_t$ &                      & 38.15         & \hphantom{0}3874.9 & 15.29 ($\times$.94)                       \\
PE-Rank                &                      & 63.54         & \hphantom{0}2949.0 & \hphantom{0}3.66 ($\times$.22)            \\ \bottomrule
\end{tabular}
\caption{Efficiency analysis or reranking top $n$ candidates retrieved by BM25 on TREC DL20.}
\label{tab:efficiency_dl20}
\end{table}

==> tables/hyperparameters.tex <==
\begin{table}[t]
\centering
\begin{tabular}{@{}lcc@{}}
\toprule
\textbf{Hyperparameter}     & \textbf{Alignment} & \textbf{LTR} \\ \midrule
optimizer                   & AdamW              & AdamW                     \\
learning rate               & 1e-4               & 2e-5                      \\
lr scheduler type           & cosine             & cosine                    \\
warmup ratio                & 0.03               & 0.03                      \\
weight dacay                & 0                  & 0                         \\
epochs                      & 1                  & 1                         \\
batch size per GPU          & 32                 & 4                         \\
gradient accumulation       & 1                  & 2                         \\
max sequence length         & 512                & 2048                      \\ \bottomrule
\end{tabular}
\caption{Hyperparameters for Training.}\label{tab:hyperparameters}
\end{table}

==> tables/sensitivity.tex <==
\begin{table}[t]
\centering
\small
\begin{tabular}{@{}l|l|cc@{}}
\toprule
\textbf{Model}  & \textbf{Order} & \textbf{TREC DL19}  & \textbf{TREC DL20}  \\
\midrule
BM25 & - & 50.58 & 47.96 \\
\midrule
\multirow{3}{*}{$\text{RankMistral}_p$} & Origin  & 71.73 & 68.07 \\
                                        & Random  & 71.04 & 67.91 \\
                                        & Inverse & 70.92 & 68.85 \\
\midrule
\multirow{3}{*}{PE-Rank}                & Origin  & 70.48 & 63.54 \\
                                        & Random  & 66.74 & 56.14 \\
                                        & Inverse & 57.15 & 49.85 \\
\bottomrule
\end{tabular}
\caption{Sensitivity to the initial ranking.}
\label{tab:sensitivity}
\end{table}

==> tables/token_analysis.tex <==
\begin{table}[t]
\centering
\small
\begin{tabular}{@{}l|cc@{}}
\toprule
    & \textbf{\# Processed} & \textbf{\# Generated} \\ \midrule
$\text{RankMistral}_{p}$ & $\mathcal{O}(L_I + n L_p)$ & $\Omega(mn)$          \\
PE-Rank                  & $\mathcal{O}(L_I + n)$     & $n$  \\ \bottomrule
\end{tabular}
\caption{Theoretical analysis on the numbers of processed and generated tokens for different methods.}
\label{tab:tokens}
\end{table}

==> tables/training_and_input.tex <==
\begin{table}[t]
\centering
\small
\begin{tabular}{@{}c|l|c|cc@{}}
\toprule
\textbf{\textit{Ret.}} & \textbf{Training Loss}  & \textbf{Input} & \textbf{DL19} & \textbf{DL20} \\
\midrule
\multirow{6}{*}{BM25} & $\mathcal{L}_{\text{rank}}$                                                          & E + T        & 65.88         & 56.67         \\
                      & $\mathcal{L}_{\text{rank}}$                                                          & E            & 68.43         & 64.42         \\
                      & $\mathcal{L}_{\text{rank}} + \mathcal{L}_{\text{content}}$                           & E + T        & 72.14         & 67.61         \\
                      & $\mathcal{L}_{\text{rank}} + \mathcal{L}_{\text{content}}$                           & E            & 68.43         & 64.03         \\
                      & $\mathcal{L}_{\text{rank}} + \mathcal{L}_{\text{content}} + \mathcal{L}_{\text{KL}}$ & E + T        & 71.16         & 64.69         \\
                      & $\mathcal{L}_{\text{rank}} + \mathcal{L}_{\text{content}} + \mathcal{L}_{\text{KL}}$ & E            & 70.48         & 63.54         \\
\midrule
\multirow{6}{*}{Jina} & $\mathcal{L}_{\text{rank}}$                                                          & E + T        & 67.20         & 66.83         \\
                      & $\mathcal{L}_{\text{rank}}$                                                          & E            & 71.17         & 69.12         \\
                      & $\mathcal{L}_{\text{rank}} + \mathcal{L}_{\text{content}}$                           & E + T        & 73.12         & 75.02         \\
                      & $\mathcal{L}_{\text{rank}} + \mathcal{L}_{\text{content}}$                           & E            & 70.51         & 70.62         \\
                      & $\mathcal{L}_{\text{rank}} + \mathcal{L}_{\text{content}} + \mathcal{L}_{\text{KL}}$ & E + T        & 71.47         & 71.73         \\
                      & $\mathcal{L}_{\text{rank}} + \mathcal{L}_{\text{content}} + \mathcal{L}_{\text{KL}}$ & E            & 70.91         & 69.48         \\
\bottomrule
\end{tabular}
\caption{}
\label{tab:training_and_input}
\end{table}

==> tables/trec.tex <==
% \begin{table*}[t]
% \centering
% \small
% \caption{Results on TREC DL.}
% \label{tab:trec}
% \begin{tabular}{@{}lc|ccc|ccc@{}}
% \toprule
% \multirow{2}{*}{\textbf{Model}} &
%   \multirow{2}{*}{\textbf{Retriever}} &
%   \multicolumn{3}{c|}{\textbf{TREC DL 19}} &
%   \multicolumn{3}{c}{\textbf{TREC DL 20}} \\
%  &
%    &
%   \textbf{NDCG@10} &
%   \textbf{\#Tokens} &
%   \textbf{Latency (ms)} &
%   \textbf{NDCG@10} &
%   \textbf{\#Tokens} &
%   \textbf{Latency (ms)} \\ \midrule
% BM25                     & -                     & 50.58 & - & - & 47.96 & - & - \\
% monoBERT                 & \multirow{4}{*}{BM25} & 70.50 & - & - & 67.28 & - & - \\
% monoT5                   &                       & 71.83 & - & - & 68.89 & - & - \\
% $\text{RankGPT}_{3.5}$   &                       & 65.80 & - & - & 62.91 & - & - \\
% $\text{RankGPT}_{4}$     &                       & 75.59 & - & - & 70.56 & - & - \\ \midrule
% $\text{RankMistral}_{p}$ & \multirow{4}{*}{BM25} & 71.73 &   &   & 68.07 &   &   \\
% $\text{RankMistral}_{s}$ &                       & 69.79 &   &   & 67.01 &   &   \\
% $\text{RankMistral}_{t}$ &                       & 45.29 &   &   & 36.87 &   &   \\
% embedding                &                       & 70.48 &   &   & 63.54 &   &   \\ \midrule
% Jina-Embeddings          & -                     & 65.94 & - & - & 63.89 & - & - \\
% $\text{RankMistral}_{p}$ & \multirow{4}{*}{Jina} & 71.44 &   &   & 73.27 &   &   \\
% $\text{RankMistral}_{s}$ &                       & 67.51 &   &   & 70.59 &   &   \\
% $\text{RankMistral}_{t}$ &                       & 42.49 &   &   & 35.32 &   &   \\
% embedding                &                       & 70.91 &   &   & 69.48 &   &   \\ \bottomrule
% \end{tabular}
% \end{table*}

\begin{table}[t]
\centering
\small
\begin{tabular}{@{}lccc@{}}
\toprule
\textbf{Model}           & \textbf{Retriever}    & \textbf{DL19} & \textbf{DL20} \\ \midrule
BM25                     & -                     & 50.58         & 47.96         \\
monoBERT                 & \multirow{7}{*}{BM25} & 70.50         & 67.28         \\
monoT5                   &                       & 71.83         & 68.89         \\ \midrule
RankVicuna               & \multicolumn{1}{l}{}  & 66.82         & 65.49         \\
RankZephyr               & \multicolumn{1}{l}{}  & 74.20         & 70.86         \\
Rank-wo-GPT              & \multicolumn{1}{l}{}  & 71.80         & 67.40         \\ \midrule
$\text{RankGPT}_{3.5}$   &                       & 65.80         & 62.91         \\
$\text{RankGPT}_{4}$     &                       & \textbf{75.59}& \textbf{70.56}\\ \midrule
$\text{RankMistral}_{p}$ & \multirow{4}{*}{BM25} & 71.73         & 68.07         \\
$\text{RankMistral}_{s}$ &                       & 69.79         & 67.01         \\
$\text{RankMistral}_{t}$ &                       & 45.29         & 36.87         \\
embedding                &                       & 70.48         & 63.54         \\ \midrule
Jina-Embeddings          & -                     & 65.94         & 63.89         \\
$\text{RankMistral}_{p}$ & \multirow{4}{*}{Jina} & 71.44         & 73.27         \\
$\text{RankMistral}_{s}$ &                       & 67.51         & 70.59         \\
$\text{RankMistral}_{t}$ &                       & 42.49         & 35.32         \\
embedding                &                       & 70.91         & 69.48         \\ \bottomrule
\end{tabular}
\caption{Results (NDCG@10) of reranking top-100 passages on TREC DL. For results in the first block, we directly copied results from~\citet{sun2023rankgpt}.}
\label{tab:trec}
\end{table}


